DS-Fusion: Artistic Typography via Discriminated and Stylized Diffusion

We introduce a novel method to automatically generate an artistic typography by stylizing one or more letter fonts to visually convey the semantics of an input word, while ensuring that the output remains readable. To address an assortment of challenges with our task at hand including conflicting goals (artistic stylization vs. legibility), lack of ground truth, and immense search space, our approach utilizes large language models to bridge texts and visual images for stylization and build an unsupervised generative model with a diffusion model backbone. Specifically, we employ the denoising generator in Latent Diffusion Model (LDM), with the key addition of a CNN-based discriminator to adapt the input style onto the input text. The discriminator uses rasterized images of a given letter/word font as real samples and output of the denoising generator as fake samples. Our model is coined DS-Fusion for discriminated and stylized diffusion. We showcase the quality and versatility of our method through numerous examples, qualitative and quantitative evaluation, as well as ablation studies. User studies comparing to strong baselines including CLIPDraw and DALL-E 2, as well as artist-crafted typographies, demonstrate strong performance of DS-Fusion.

==> figs/fig_ablation_nomse.tex <==
\begin{figure}
\centering
  \includegraphics[width=0.99\columnwidth]{data/ablation_nomse.pdf}
  \caption{Effect of not using diffusion loss: From epochs 180 to 300. It loses the information of style and converges to the glyph only.}
  \label{fig:ablation_nomse}
\end{figure}

==> figs/fig_ablation_prompt.tex <==
\begin{figure}
\centering
  \includegraphics[width=0.99\columnwidth]{data/ablation_prompt.pdf}
  \caption{\yw{Effect of using different \rz{conditioning} prompts on style CAT and glyph C. The left column demonstrates different conditioning prompts, where ``Random'' refers to a random five-character string. The number below each image denotes the training epoch.} }
  \label{fig:alblation_prompt}
\end{figure}
% The epochs under the images show the speed of convergence in each case.

==> figs/fig_extension.tex <==
\begin{figure}
\centering
  \includegraphics[width=0.99\columnwidth]{data/results_extensions.pdf}
  \caption{Extension to other objects.}
  \label{fig:res_extensions}
\end{figure}

==> figs/fig_res_qual_single_letter.tex <==
\begin{figure*}
\centering
  \includegraphics[width=0.99\textwidth]{data/results_single_letter}
  \caption{Stylizing single letters.}
  \label{fig:res_qual_single_letter}
\end{figure*}

==> tables/tab_ablation.tex <==
\begin{table}
	\centering
	\begin{tabular}{lrr}
	\toprule
        Setting & MSE$\downarrow$ & CLIP $\uparrow$    \\
		\midrule
         w/o Dis     &  &  \\
         w/o $l_{rec}$   &  &    \\
         CLIP   &  &    \\
         Full    &    & \\
		\bottomrule
	\end{tabular}

  	\caption{Abaltion Studies.}

    \label{tab:ablation}
\end{table}

==> tables/tab_eval_multfont.tex <==
\begin{table}
	\centering
	\begin{tabular}{lccc}
	\toprule
        Method & OCR$\uparrow$ & OCR [blur] $\uparrow$   & CLIP $\uparrow$  \\
		\midrule
             CLIPDraw~\cite{frans2021clipdraw} & 4.6 &   11.4 &  23.9\\
             \yw{DS-Fusion}  &  5.3 & 22.0 & 24.0\\
		\bottomrule
	\end{tabular}

  	\caption{\yw{Quantitative comparison between CLIPDraw and DS-Fusion when }\mt{using multiple fonts as input.}}

    \label{tab:eval_all_font}
\end{table}


==> tables/tab_eval_quan.tex <==
\resizebox{\columnwidth}{!}
\begin{table}

	\centering
	\begin{tabular}{lrrr}
	\toprule
        Method & CLIP Letter$\uparrow$ & CLIP Style $\uparrow$  & User $\uparrow$  \\
		\midrule
             DALL-E 2~\cite{ramesh2022hierarchical} &  &  &  \\
             SD~\cite{rombach2022high}  &  & &  \\
             CLIPDraw~\cite{frans2021clipdraw} &  &   &   \\
             %DF-GAN~\cite{wang2022diffusion} &  &  &    \\
             Google Search &  &  &  \\
             Ours  &  &  & \\
		\bottomrule
	\end{tabular}

  	\caption{One-Font Comparison}

    \label{tab:eval_quan_abc}
\end{table}


==> tables/tab_user_study_vs_human.tex <==
\begin{table}
	\centering
	\begin{tabular}{lccc}
	\toprule
         Human & Equal & DS-Fusion \\
		\midrule
             56.75 & 10.0 &  32.25 \\
		\bottomrule
	\end{tabular}

  	\caption{\yw{User study comparing results from DS-Fusion and human designers. The numbers show the percentage of user preference for different methods. }}

    \label{tab:eval_user_study_vs_human}
\end{table}
